(Mis)Fitting: A Survey of Scaling Laws

Modern foundation models rely heavily on using scaling laws to guide crucial training decisions. Researchers often extrapolate the optimal architecture and hyper parameters settings from smaller training runs by describing the relationship between, loss, or task performance, and scale. All components of this process vary, from the specific equation being fit, to the training setup, to the optimization method. Each of these factors may affect the fitted law, and therefore, the conclusions of a given study. We discuss discrepancies in the conclusions that several prior works reach, on questions such as the optimal token to parameter ratio. We augment this discussion with our own analysis of the critical impact that changes in specific details may effect in a scaling study, and the resulting altered conclusions. Additionally, we survey over 50 papers that study scaling trends: while 45 of these papers quantify these trends using a power law, most under-report crucial details needed to reproduce their findings. To mitigate this, we we propose a checklist for authors to consider while contributing to scaling law research.

==> images/analysis_fig_main.tex <==


\begin{figure}[!h]
\centering

\begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/analysis_nd_ours_C_vs_N.png}
    \caption{\textbf{\S\ref{sec:model_training}, \S\ref{sec:repl-model_training}} Of the models we train, we choose subsets with ($N$, $D$) values which fit a particular method one might have of setting up training. Results vary dramatically between settings.}
    \label{fig:analysis_nd_ours_main}
\end{subfigure}
\hfill
\begin{subfigure}{0.47\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/analysis_counting_ours_C_vs_N.png}
    \caption{\textbf{\S\ref{sec:model_training}, \S\ref{sec:repl-model_training}} We fit power laws to our models and vary the ways we count $N$ and $C$, including or excluding embeddings, as well as using the $C=6ND$ approximation.
    The difference in resulting scaling laws is substantial and increases with scale. 
    }
    \label{fig:analysis_counting_ours_main}
\end{subfigure}


\begin{subfigure}{\textwidth}
\begin{subfigure}{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/analysis_init_epoch_ai_C_vs_N.png}
    % \caption{Initialization schemes, epochs}
    % \label{fig:analysis_init_epoch}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/analysis_init_ours_C_vs_N.png}
    % \caption{Inits, ours}
    % \label{fig:analysis_init_ours}
\end{subfigure}
\caption{\textbf{\S\ref{sec:opt}, \S\ref{sec:repl-opt}} We fit to data from \citet{besiroglu2024chinchilla} (left) and our data (right) to experiment with the initialization of parameters in the power law. Results do not follow a clear pattern and are unstable, suggesting the difficulty of optimizing over this space, and the presence of many local minima.
}
\label{fig:analysis_init_main}
\end{subfigure}

\caption{(\textbf{\S\ref{sec:own-repl}}) We study the effects of various decisions in the fitting of a power law, as outlined in our checklist (Appendix~\ref{sec:app_checklist}) and detailed in \S\ref{sec:power-law-form}-\S\ref{sec:opt}. For comparison, we include Llama 3 405B \citep{dubey2024llama}, the Chinchilla model \citep{hoffmann2022training}, and an estimate of the 1.5B GPT-2 model \citep{radford2019language}, as well as the \citep{kaplan2020scaling} and \citep{hoffmann2022training} scalig laws. A thick, solid line indicates lowest optimization loss in each plot. Overall, these choices strongly affect the power law fit. Thorough reporting of these decisions may be critical for scaling law reproducibility.
}
\label{fig:overall}
\end{figure}

==> sections/preliminaries.tex <==

% \section{Preliminaries}\label{sec:method}
%  \srk{TO REMOVE}
% \subsection{Power Laws for Large Models}

% \srk{this does is repeated in Section 5 - maybe remove? but how to remove?}
% % What are power laws, where else are they used, how are they usually fit, what kinds of forms do they take? 


% It has become common to characterize the loss of large foundation models by using a power law.

% \[  f(x)=ax^{-k} \]

% In this section we will describe things specifically for transformer language models, but in Section \ref{sec:power-law-form}, we go further into which forms other papers have considered to answer specific research questions for different modalities and architecture families. 

% In its most simple form, one can consider a model for size $N$ trained for $D$ tokens and find that the loss for the model can be described as a power law in both $N$ and $D$. That is, 

% \[ L \propto N^a , L \propto D^a \]

% These are often combined to fit a single equation in terms of both $N$ and $D$. For example, \cite{hoffmann2022training} use the following equation

% \[ L(N, D) = E + \frac{A}{N^{\alpha}} + \frac{B}{D^{\beta}} \]

% \subsection{Models}

% \srk{honestly not sure what to do with this section either}




% Maybe stuff like what is a token, what is a FLOP / how do you calculate FLOPs, what is embedding vs non embedding parameters, what is test loss?


==> tables/checklist.tex <==
\fbox{\begin{minipage}{38em}

\subsubsection*{Scaling Law Reproducilibility Checklist}\label{sec:checklist}


\small

\begin{minipage}[t]{0.48\textwidth}
\raggedright
\paragraph{Scaling Law Hypothesis (\S\ref{sec:power-law-form})}

\begin{itemize}[leftmargin=*]
    \item What is the form of the power law?
    \item What are the variables related by (included in) the power law?
    \item What are the parameters to fit?
    \item On what principles is this form derived?
    \item Does this form make assumptions about how the variables are related?
    % \item How are each of these variables counted? (For example, how is compute cost/FLOPs counted, if applicable? How are parameters of the model counted?)
    % \item Are code/code snippets provided for calculating these variables if applicable? 
\end{itemize}


\paragraph{Training Setup (\S\ref{sec:model_training})}
\begin{itemize}[leftmargin=*]
    \item How many models are trained?
    \item At which sizes?
    \item On how much data each? On what data? Is any data repeated within the training for a model?
    \item How are model size, dataset size, and compute budget size counted? For example, how are parameters of the model counted? Are any parameters excluded (e.g., embedding layers)?
    \item Are code/code snippets provided for calculating these variables if applicable?
    % embedding  For example, how is compute cost counted, if applicable? 
    \item How are hyperparameters chosen (e.g., optimizer, learning rate schedule, batch size)? Do they change with scale?
    \item What other settings must be decided (e.g., model width vs. depth)? Do they change with scale?
    \item Is the training code open source?
    % \item How is the correctness of the scaling law considered SHOULD WE?
\end{itemize}

\end{minipage}
\begin{minipage}[t]{0.48\textwidth}
\raggedright


\paragraph{Data Collection(\S\ref{sec:data})}
\begin{itemize}[leftmargin=*]
    \item Are the model checkpoints provided openly?
    % \item Are these checkpoints modified in any way before evaluation? (say, checkpoint averaging)
    % \item If the above is done, is code for modifying the checkpoints provided?
    \item How many checkpoints per model are evaluated to fit each scaling law?
    \item What evaluation metric is used? On what dataset?
    \item Are the raw evaluation metrics modified, e.g., through loss interpolation, centering around a mean, scaling logarithmically, etc?
    \item If the above is done, is code for modifying the metric provided? 
\end{itemize}

\paragraph{Fitting Algorithm (\S\ref{sec:opt})}
\begin{itemize}[leftmargin=*]
    \item What objective (loss) is used?
    \item What algorithm is used to fit the equation?
    \item What hyperparameters are used for this algorithm?
    \item How is this algorithm initialized?
    \item Are all datapoints collected used to fit the equations? For example, are any outliers dropped? Are portions of the datapoints used to fit different equations?
    \item How is the correctness of the scaling law considered? Extrapolation, Confidence Intervals, Goodness of Fit?
\end{itemize}

\end{minipage}

% \paragraph{Other}
% \begin{itemize}
%     \item Is code for 
% \end{itemize}

\end{minipage}}
